A Benchmark and a Baseline for Robust Multi-view Depth Estimation

Recent deep learning approaches for multi-view depth estimation are employed either in a depth-from-video or a multi-view stereo setting. Despite different settings, these approaches are technically similar: they correlate multiple source views with a keyview to estimate a depth map for the keyview. In this work, we introduce the Robust Multi-View Depth Benchmark that is built upon a set of public datasets and allows evaluation in both settings on data from different domains. We evaluate recent approaches and find imbalanced performances across domains. Further, we consider a third setting, where camera poses are available and the objective is to estimate the corresponding depth maps with their correct scale. We show that recent approaches do not generalize across datasets in this setting. This is because their cost volume output runs out of distribution. To resolve this, we present the Robust MVD Baseline model for multi-view depth estimation, which is built upon existing components but employs a novel scale augmentation procedure. It can be applied for robust multi-view depth estimation, independent of the target data. We provide code for the proposed benchmark and baseline model at https://github.com/lmb-freiburg/robustmvd.

==> 000_header.tex <==
% Include other packages here, before hyperref.
\RequirePackage[format=plain,labelformat=simple,labelsep=period,font=small,compatibility=false]{caption}
\RequirePackage[font=footnotesize,skip=3pt,subrefformat=parens]{subcaption}

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{times}
\usepackage{epsfig}
% \usepackage{adjcalc}
% \usepackage{adjustbox}
\usepackage{pifont}
\usepackage{color, colortbl}
\usepackage{siunitx}
% \usepackage{subfig}
% \usepackage{bm}
\usepackage[table]{xcolor} % for coloring cells
\usepackage[inline]{enumitem}
% \usepackage{blindtext}
% \usepackage{lipsum}
% \usepackage{mathtools}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{xr-hyper}
\usepackage{pdfpages}
\include{enumitem}


% It is strongly recommended to use hyperref, especially for the review version.
% hyperref with option pagebackref eases the reviewers' job.
% Please disable hyperref *only* if you encounter grave issues, e.g. with the
% file validation for the camera-ready version.
%
% If you comment hyperref and then uncomment it, you should delete
% ReviewTempalte.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).
\usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}


% Support for easy cross-referencing
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

% colors:
\definecolor{mylightgreen}{RGB}{51,153,102}
\definecolor{mydarkgreen}{RGB}{17,121,74}

\definecolor{mygreenblue}{RGB}{47,111,112}
\definecolor{mylightblue}{RGB}{172,207,208} 

\definecolor{myyellow}{RGB}{215,179,18} 
\definecolor{myorange}{RGB}{215,136,18}

\definecolor{mylightred}{RGB}{192,72,72} 
\definecolor{mydarkred}{RGB}{158,28,28} 

\definecolor{mylightgray}{RGB}{238,238,238} 
\definecolor{mymedgray}{RGB}{202,204,206} 
\definecolor{mydarkgray}{RGB}{42,44,46}

\definecolor{mymaxturbo}{RGB}{161,17,1}
\definecolor{myminturbo}{RGB}{57,42,119}

\colorlet{bgcolor}{mylightgray}
\colorlet{poscolor}{mydarkgreen}
\colorlet{negcolor}{mydarkred}
\colorlet{outputscalingcolor}{blue}
\definecolor{draftcolor}{RGB}{0,73,95}

% comment commands:
\newcommand{\tb}[1]{\textcolor{mydarkgreen}{\footnotesize Thomas: #1}} % Thomas comments
\newcommand{\tcb}[1]{\textcolor{mydarkgreen}{\footnotesize Thomas: #1}} % Thomas comments
\newcommand{\tcp}[1]{\textcolor{mydarkred}{\footnotesize Philipp: #1}} % Philipp comments
\newcommand{\cz}[1]{\textcolor{mygreenblue}{\footnotesize Christian: #1}} % Christian comments
\newcommand{\tco}[1]{\textcolor{myorange}{\footnotesize Ozgun: #1}} % Ozgun comments
\newcommand{\ar}[1]{\textcolor{mygreenblue}{\footnotesize Artemij: #1}} % Christian comments
\newcommand{\jan}[1]{\textcolor{mylightgreen}{\footnotesize Jan: #1}} % Jan comments

% \newcommand{\tb}[1]{\textcolor{mydarkgreen}{}} % Thomas comments
% \newcommand{\tcb}[1]{\textcolor{mydarkgreen}{}} % Thomas comments
% \newcommand{\tcp}[1]{\textcolor{mydarkred}{}} % Philipp
% \newcommand{\cz}[1]{\textcolor{mygreenblue}{}} % Christian comments
% \newcommand{\tco}[1]{\textcolor{myorange}{}} % Ozgun comments
% \newcommand{\ar}[1]{\textcolor{mygreenblue}{}} % Christian comments
% \newcommand{\jan}[1]{\textcolor{mylightgreen}{}} % Jan comments

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newcommand{\tdraft}[1]{\textcolor{draftcolor}{Draft: #1}}
\newcommand{\ttodo}[1]{\textcolor{mydarkred}{Todo: #1}}

% custom commands:
\newcommand{\deeplearningcluster}{Gef\"ordert durch die Deutsche Forschungsgemeinschaft (DFG) - 417962828} 
\newcommand{\deeplearningclusterEN}{Funded by the Deutsche Forschungsgemeinschaft (DFG) - 417962828} 
\newcommand{\fakeparagraph}[1]{\noindent\textbf{#1}{ }}

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norm}[2]{\left\lVert #1 \right\rVert_{#2}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\vect}[1]{\mathbf{#1}}
% \newcommand{\my}{\textcolor{poscolor}{\ding{51}}}
% \newcommand{\mn}{\textcolor{negcolor}{\ding{51}}}
\newcommand{\my}{\ding{51}}
\newcommand{\mn}{\ding{55}}
\newcommand{\bb}[1]{\textbf{#1}}
\def\rot#1{\rotatebox{90}{#1}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

% placeholders:
\newcommand{\ourapproach}{DistNet}
\hyphenation{DistNet}

% math placeholders naming scheme:
    % -set of sets: mathcal
    % -set/tuple: uppercase
    % -matrix: uppercase, bold
    % -vector: lowercase, bold
    % scalar: lowercase
    % function (e.g. neural network): lowercase (or uppercase?)

\newcommand{\other}{source}
\newcommand{\Other}{Source}
\newcommand{\Otherview}{\Other{} view}
\newcommand{\otherview}{\other{} view}
\newcommand{\otherviews}{\otherview{}s}
\newcommand{\key}{key}
\newcommand{\Key}{Key}
\newcommand{\keyview}{keyview}
\newcommand{\keyviews}{keyviews}

\newcommand{\sethree}{SE(3)}
\newcommand{\sothree}{SO(3)}
\newcommand{\realnumbers}{\mathbb{R}}
\newcommand{\projectivespace}{\mathbb{P}}

\newcommand{\fromto}[2]{{}^{#1}_{#2}}
\newcommand{\coordsin}[2]{{}^{#1}{#2}}
\newcommand{\homog}[1]{\tilde{#1}}
\newcommand{\scaledshifted}[1]{\hat{#1}}
\newcommand{\scaledshiftedin}[2]{\coordsin{#1}{\scaledshifted{#2}}}

\newcommand{\testsets}{\mathcal{D}}
\newcommand{\testset}{D}
\newcommand{\sample}{S}
\newcommand{\sampleinput}{V}
\newcommand{\labels}{L}
\newcommand{\view}{V}

\newcommand{\inputwidth}{W}
\newcommand{\inputheight}{H}
\newcommand{\featurewidth}{w}
\newcommand{\featureheight}{h}
\newcommand{\featurechannels}{c}
\newcommand{\correlationsteps}{n}

\newcommand{\image}{\mathbf{I}}
\newcommand{\featuremap}{\mathbf{F}}
\newcommand{\ctxfeaturemap}{\mathbf{\hat{F}}}
\newcommand{\feature}{\mathbf{f}}
\newcommand{\intrinsic}{\mathbf{K}}
\newcommand{\costvolume}{\textbf{C}}
% \newcommand{\encoder}{f}
% \newcommand{\fusion}{g}
% \newcommand{\decoder}{h}
% \newcommand{\ctx}{k}
\newcommand{\encoder}{f_{\theta}}
\newcommand{\fusion}{g_{\rho}}
\newcommand{\ctx}{h_{\sigma}}
\newcommand{\decoder}{k_{\phi}}
\newcommand{\uncertaintydecoder}{l_{\psi}}
\newcommand{\simfct}{sim}

\newcommand{\transform}{\mathbf{T}}
\newcommand{\translation}{\mathbf{t}}
\newcommand{\rotation}{\mathbf{R}}
\newcommand{\transformfromto}[2]{\fromto{#1}{#2}\transform}
\newcommand{\translationfromto}[2]{\fromto{#1}{#2}\translation}
\newcommand{\rotationfromto}[2]{\fromto{#1}{#2}\rotation}

% uncertainty:
\newcommand{\uncertaintymap}{\mathbf{U}}  % 2d matrix of depth values

% depth:
\newcommand{\depthval}{z}
\newcommand{\depths}{\mathbf{\depthval}}  % vector of depth values
\newcommand{\depthmap}{\mathbf{Z}}  % 2d matrix of depth values

\newcommand{\preddepthval}{\depthval}
\newcommand{\preddepths}{\depths}
\newcommand{\preddepthmap}{\depthmap}
\newcommand{\preddepthsscaled}{\hat{\preddepths}}  % or\mathbf{\hat{z}}
\newcommand{\preddepthmapscaled}{\hat{\preddepthmap}}  % or\mathbf{\hat{z}}

\newcommand{\gtdepthval}{\depthval^\ast}
\newcommand{\gtdepths}{\depths^\ast}  % or \mathbf{\gtdepthval} 
\newcommand{\gtdepthmap}{\depthmap^\ast}

%invdepth:
\newcommand{\invdepthval}{d}
\newcommand{\invdepths}{\mathbf{\invdepthval}}  % vector of invdepth values
\newcommand{\invdepthmap}{\mathbf{D}}  % 2d matrix of invdepth values
\newcommand{\invdepthvalin}[1]{\coordsin{#1}{\invdepthval}}

\newcommand{\predinvdepthval}{\invdepthval}
\newcommand{\predinvdepths}{\invdepths}
\newcommand{\predinvdepthmap}{\invdepthmap}

\newcommand{\gtinvdepthval}{\invdepthval^\ast}
\newcommand{\gtinvdepths}{\invdepths^\ast}  % or \mathbf{\gtinvdepthval}
\newcommand{\gtinvdepthmap}{\invdepthmap^\ast}

% disparity:
\newcommand{\dispmap}{\bm{\Delta}}
\newcommand{\dispmapin}[1]{\coordsin{#1}\dispmap}

\newcommand{\disp}{\bm{\delta}}
\newcommand{\homogdisp}{\homog{\bm{\Delta}}}
\newcommand{\dispin}[1]{\coordsin{#1}\disp}
\newcommand{\homogdispin}[1]{\coordsin{#1}\homogdisp}

\newcommand{\dispval}{\delta}
\newcommand{\homogdispval}{\homog{\mathbf{m}}}
\newcommand{\dispvalin}[1]{\coordsin{#1}\dispval}
\newcommand{\homogdispvalin}[1]{\coordsin{#1}\homogdispval}
\newcommand{\gtdispval}{\dispval^\ast}
\newcommand{\gtdispvalin}[1]{\coordsin{#1}\gtdispval}

\newcommand{\dispvalx}{\dispval_{\pointtwodx}}
\newcommand{\dispgradx}{\dispvalx'}
\newcommand{\homogdispvalx}{\homog{m_{\pointtwodx}}}
\newcommand{\dispvalxin}[1]{\coordsin{#1}\dispvalx}
\newcommand{\dispgradxin}[1]{\coordsin{#1}\dispgradx}
\newcommand{\homogdispvalxin}[1]{\coordsin{#1}\homogdispvalx}

\newcommand{\dispvaly}{\dispval_{\pointtwody}}
\newcommand{\dispgrady}{\dispvaly'}
\newcommand{\homogdispvaly}{\homog{m_{\pointtwody}}}
\newcommand{\dispvalyin}[1]{\coordsin{#1}\dispvaly}
\newcommand{\dispgradyin}[1]{\coordsin{#1}\dispgrady}
\newcommand{\homogdispvalyin}[1]{\coordsin{#1}\homogdispvaly}

\newcommand{\dispvalz}{\dispval_{\pointtwodz}}
\newcommand{\homogdispvalz}{\homog{m_{\pointtwodz}}}
\newcommand{\dispvalzin}[1]{\coordsin{#1}\dispvalz}
\newcommand{\homogdispvalzin}[1]{\coordsin{#1}\homogdispvalz}

% points in 2d and 3d:

\newcommand{\pointthreed}{\mathbf{X}}
\newcommand{\pointthreedin}[1]{\coordsin{#1}{\pointthreed}}
\newcommand{\homogpointthreed}{\homog{\pointthreed}}
\newcommand{\homogpointthreedin}[1]{\coordsin{#1}{\homogpointthreed}}

\newcommand{\pointthreedx}{x}
\newcommand{\pointthreedxin}[1]{\coordsin{#1}{\pointthreedx}}
\newcommand{\pointthreedy}{y}
\newcommand{\pointthreedyin}[1]{\coordsin{#1}{\pointthreedy}}
\newcommand{\pointthreedz}{z}
\newcommand{\pointthreedzin}[1]{\coordsin{#1}{\pointthreedz}}

\newcommand{\pointtwod}{\mathbf{x}}
\newcommand{\pointtwodin}[1]{\coordsin{#1}{\pointtwod}}
\newcommand{\homogpointtwod}{\homog{\pointtwod}}
\newcommand{\homogpointtwodin}[1]{\coordsin{#1}{\homogpointtwod}}

\newcommand{\pointtwodx}{u}
\newcommand{\pointtwodxin}[1]{\coordsin{#1}{\pointtwodx}}
\newcommand{\homogpointtwodx}{\homog{\pointtwodx}}
\newcommand{\homogpointtwodxin}[1]{\coordsin{#1}{\homogpointtwodx}}
\newcommand{\pointtwody}{v}
\newcommand{\pointtwodyin}[1]{\coordsin{#1}{\pointtwody}}
\newcommand{\homogpointtwody}{\homog{\pointtwody}}
\newcommand{\homogpointtwodyin}[1]{\coordsin{#1}{\homogpointtwody}}
\newcommand{\pointtwodz}{k}
\newcommand{\homogpointtwodz}{\homog{\pointtwodz}}
\newcommand{\homogpointtwodzin}[1]{\coordsin{#1}{\homogpointtwodz}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pointalpha}{\mathbf{\pmb{\alpha}}}
\newcommand{\pointalphain}[1]{\coordsin{#1}{\pointalpha}}

\newcommand{\pointalphax}{\alpha_\pointtwodx}
\newcommand{\pointalphaxin}[1]{\coordsin{#1}{\pointalphax}}
\newcommand{\pointalphay}{\alpha_\pointtwody}
\newcommand{\pointalphayin}[1]{\coordsin{#1}{\pointalphay}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pointtwodinf}{\pointtwod_{\infty}}
\newcommand{\pointtwodinfin}[1]{\coordsin{#1}{\pointtwodinf}}
\newcommand{\homogpointtwodinf}{\homog{\pointtwod}_{\infty}}
\newcommand{\homogpointtwodinfin}[1]{\coordsin{#1}{\homogpointtwodinf}}

\newcommand{\pointtwodinfx}{\pointtwodx_{\infty}}
\newcommand{\pointtwodinfxin}[1]{\coordsin{#1}{\pointtwodinfx}}
\newcommand{\homogpointtwodinfx}{\homog{\pointtwodx}_{\infty}}
\newcommand{\homogpointtwodinfxin}[1]{\coordsin{#1}{\homogpointtwodinfx}}

\newcommand{\pointtwodinfy}{\pointtwody_{\infty}}
\newcommand{\pointtwodinfyin}[1]{\coordsin{#1}{\pointtwodinfy}}
\newcommand{\homogpointtwodinfy}{\homog{\pointtwody}_{\infty}}
\newcommand{\homogpointtwodinfyin}[1]{\coordsin{#1}{\homogpointtwodinfy}}

\newcommand{\pointtwodinfz}{\pointtwodz_{\infty}}
\newcommand{\pointtwodinfzin}[1]{\coordsin{#1}{\pointtwodinfz}}
\newcommand{\homogpointtwodinfz}{\homog{\pointtwodz}_{\infty}}
\newcommand{\homogpointtwodinfzin}[1]{\coordsin{#1}{\homogpointtwodinfz}}

% shifts and scales:
\newcommand{\scalingfactor}{\alpha}
\newcommand{\shift}{b}
\newcommand{\scalingfactorin}[1]{\coordsin{#1}{\scalingfactor}}
\newcommand{\shiftin}[1]{\coordsin{#1}{\shift}}
\newcommand{\scalemap}{\mathbf{A}}
\newcommand{\shiftmap}{\mathbf{B}}

% metrics:
\newcommand{\ausename}{Area Under Sparsification Error Curve}
\newcommand{\ause}{\textrm{AUSE}}
\newcommand{\absrelname}{Absolute Relative Error}
% \newcommand{\absrel}{AbsRel}
\newcommand{\absrel}{\textrm{rel}}
\newcommand{\sqrel}{SqRel}
\newcommand{\sqrelsign}{SqRel}
\newcommand{\rmse}{RMSE}
\newcommand{\rmsesign}{RMSE}
\newcommand{\rmselog}{RMSElog}
\newcommand{\rmselogsign}{RMSElog}
\newcommand{\threshIname}{Inlier Ratio}% with a threshold of $1.25$}
% \newcommand{\threshI}{\delta_{<1.25}}
\newcommand{\threshI}{\tau}
\newcommand{\threshII}{$\delta<1.25^2$}
\newcommand{\threshIIsign}{$\delta<{1.25^2}$}
\newcommand{\threshIII}{$\delta<1.25^3$}
\newcommand{\threshIIIsign}{$\delta<{1.25^3}$}

% datasets:
\newcommand{\kitti}{KITTI}
\newcommand{\kittishort}{KITTI}
\newcommand{\megadepth}{MegaDepth}
\newcommand{\megadepthshort}{MD}
\newcommand{\redweb}{ReDWeb}
\newcommand{\redwebshort}{RW}
\newcommand{\movies}{3D Movies}
\newcommand{\moviesshort}{MV}
\newcommand{\sintel}{Sintel}
\newcommand{\sintelshort}{Sintel}
\newcommand{\diw}{Depth in the Wild}
\newcommand{\diwshort}{DIW}
\newcommand{\diml}{DIML Indoor}
\newcommand{\dimlshort}{DL}
\newcommand{\wsvd}{Web Stereo Video Dataset}
\newcommand{\wsvdshort}{WSVD}
\newcommand{\ethd}{ETH3D}
\newcommand{\ethdshort}{ETH3D}
\newcommand{\nyu}{NYUDv2}
\newcommand{\nyushort}{NYU}
\newcommand{\tumrgbd}{TUM-RGBD}
\newcommand{\tumrgbdshort}{TUM}
\newcommand{\scannet}{ScanNet}
\newcommand{\scannetshort}{ScanNet}
\newcommand{\flyingthings}{FlyingThings3D}
\newcommand{\flyingthingsshort}{FT3D}
\newcommand{\staticthings}{StaticThings3D}
\newcommand{\staticthingsshort}{ST3D}
\newcommand{\realthings}{RealThings}
\newcommand{\realthingsshort}{RT}
\newcommand{\sun}{SUN3D}
\newcommand{\sunshort}{SUN}
\newcommand{\dtu}{DTU}
\newcommand{\dtushort}{DTU}
\newcommand{\tanksandtemples}{Tanks and Temples}
\newcommand{\tanksandtemplesshort}{T\&T}
\newcommand{\blendedmvs}{BlendedMVS}
\newcommand{\blendedmvsshort}{BMVS}

\newcommand{\benchmarkname}{Robust MVD Benchmark}
\newcommand{\baselinename}{Robust MVD Baseline}


% results table:
% \newcommand{\trainedsimto}[1]{\textcolor{negcolor}{#1}}
\newcommand{\trainedsimto}[1]{(#1)}
\newcommand{\bestresult}[1]{\textbf{#1}}
\newcommand{\usesoutputscaling}[1]{\textcolor{outputscalingcolor}{#1}}
\newcommand{\worsethanmedian}[1]{\textcolor{negcolor}{#1}}

==> figures/eval_uncertainty/eval_uncertainty.tex <==
\begin{figure}[h!]
        \centering
        \subfloat[]{\includegraphics[width=0.24\linewidth]{figures/eval_uncertainty/all_combined/KittiTest_65.png}\label{subfig:eval_uncertainty-a} }
        \subfloat[]{
        \includegraphics[width=0.24\linewidth]{figures/eval_uncertainty/all_combined/ScanNetTest_1980.png}\label{subfig:eval_uncertainty-b} }
        \subfloat[]{
        \includegraphics[width=0.24\linewidth]{figures/eval_uncertainty/all_combined/ETH3DTest_62.png}\label{subfig:eval_uncertainty-c} }
        \subfloat[]{
        \includegraphics[width=0.24\linewidth]{figures/eval_uncertainty/all_combined/RealThingsTest_56.png}\label{subfig:eval_uncertainty-d}}
        \caption{\textbf{Uncertainty estimation}: the first row shows \keyview{} images, the second row predicted inverse depth maps, and the third row predicted uncertainty maps. The model outputs high uncertainties for problematic cases like \protect\subref{subfig:eval_uncertainty-a} moving objects,  \protect\subref{subfig:eval_uncertainty-b} textureless regions, \protect\subref{subfig:eval_uncertainty-c} specular surfaces, and \protect\subref{subfig:eval_uncertainty-d} thin structures.}
        \label{fig:eval_uncertainty}
\end{figure}

==> figures/teaser/teaser_new.tex <==
\begin{figure}[!ht]
\centering
\def\tmpwidth{0.3\linewidth}
\def\tmpwidthh{0.14\linewidth}
\begin{tabular}{@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{}}
    % & \multicolumn{3}{c}{\textit{Training on randomized synthetic data:}} \\
    % \makecell{\rotatebox{90}{\staticthingsshort{}}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/staticthings_0.png}} &
    % \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_m2.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_m1.png}} \\
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_1.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_2.png}} \\
    % \end{tabular}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/staticthings.png}} \\
    & \multicolumn{3}{c}{\textit{Zero-shot evaluation across domains and scales:}} \\
    \makecell{\rotatebox{90}{\kittishort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/kitti_0.png}} &
    \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/kitti_m2.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/kitti_m1.png}} \\
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/kitti_1.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/kitti_2.png}} \\
    \end{tabular}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/kitti.png}} \\
    \makecell{\rotatebox{90}{\scannetshort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/scannet_0.png}} &
    \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/scannet_m2.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/scannet_m1.png}} \\
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/scannet_1.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/scannet_2.png}} \\
    \end{tabular}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/scannet.png}} \\
    \makecell{\rotatebox{90}{\ethdshort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/eth3d_0.png}} &
    \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/eth3d_1.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/eth3d_2.png}} \\
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/eth3d_3.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/eth3d_4.png}} \\
    \end{tabular}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/eth3d.png}} \\
    \makecell{\rotatebox{90}{\tanksandtemplesshort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/tanksandtemples_0.png}} &
    \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/tanksandtemples_1.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/tanksandtemples_2.png}} \\
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/tanksandtemples_3.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/tanksandtemples_4.png}} \\
    \end{tabular}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/tanksandtemples.png}} \\
    \makecell{\rotatebox{90}{\dtu{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/dtu_0.png}} &
    \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/dtu_1.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/dtu_2.png}} \\
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/dtu_3.png}} &
        \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/dtu_4.png}} \\
    \end{tabular}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/dtu.png}} \\
    % \makecell{\rotatebox{90}{\sintelshort{}}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/sintel.png}} &
    % \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} \\
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} \\
    % \end{tabular}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/sintel.png}} \\
    & \Key{} Frame & \Other{} Frames & Prediction
\end{tabular}
\caption{We introduce the Robust Multi-View Depth Benchmark to evaluate multi-view depth estimation models regarding robust application on arbitrary real-world data. The benchmark comprises evaluation on multiple existing datasets from different domains. % against absolute depth maps at real-world scale. 
We provide a baseline model that is build on existing components and generalizes well across domains and can be applied and extended for robust multi-view depth estimation. Predictions shown above are from the baseline model on benchmark data. }
\label{fig:teaser}
\end{figure}


==> figures/teaser/teaser_viridis.tex <==
\begin{figure}[!ht]
\centering
\def\tmpwidth{0.3\linewidth}
\def\tmpwidthh{0.14\linewidth}
\begin{tabular}{@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{}}
    % & \multicolumn{3}{c}{\textit{Training on randomized synthetic data:}} \\
    % \makecell{\rotatebox{90}{\staticthingsshort{}}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/staticthings_0.png}} &
    % \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_m2.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_m1.png}} \\
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_1.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/staticthings_2.png}} \\
    % \end{tabular}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/staticthings.png}} \\
    & \multicolumn{3}{c}{\textit{Zero-shot evaluation across domains and scales:}} \\
    \makecell{\rotatebox{90}{\kittishort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/kitti_0.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/kitti.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_uncertainty_viridis/kitti.png}} \\
    \makecell{\rotatebox{90}{\scannetshort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/scannet_0.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/scannet.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_uncertainty_viridis/scannet.png}} \\
    \makecell{\rotatebox{90}{\ethdshort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/eth3d_0.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/eth3d.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_uncertainty_viridis/eth3d.png}} \\
    \makecell{\rotatebox{90}{\tanksandtemplesshort{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/tanksandtemples_0.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/tanksandtemples.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_uncertainty_viridis/tanksandtemples.png}} \\
    \makecell{\rotatebox{90}{\dtu{}}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/dtu_0.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/dtu.png}} &
    \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_uncertainty_viridis/dtu.png}} \\
    % \makecell{\rotatebox{90}{\sintelshort{}}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/images/sintel.png}} &
    % \makecell{\begin{tabular}{@{}c@{\hspace{1mm}}c@{}}
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} \\
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} &
    %     \makecell{\includegraphics[width=\tmpwidthh]{figures/teaser/images/images/sintel.png}} \\
    % \end{tabular}} &
    % \makecell{\includegraphics[width=\tmpwidth]{figures/teaser/images/pred_invdepth/sintel.png}} \\
    & \Key{} Frame & Pred. Depth & Pred. Uncertainty
\end{tabular}
\caption{We introduce the Robust Multi-View Depth (MVD) Benchmark to evaluate multi-view depth estimation models regarding robust application on arbitrary real-world data. The benchmark comprises evaluation of depth and uncertainty estimates on multiple existing datasets from different domains and includes a setting with given camera poses and evaluation against absolute depth maps at real-world scale. 
We provide a baseline model that is build on existing components and generalizes well across domains and can be applied and extended for robust multi-view depth estimation. Predictions shown above are from the baseline model on benchmark data. \textcolor{myminturbo}{Blue} colors indicate small values, \textcolor{mymaxturbo}{red} colors large values, and the ranges are given in meters.}
\label{fig:teaser}
\end{figure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}


==> tables/eval_baseline_traindata.tex <==
\begin{table*}[!t]
% \begin{table}[t]
\scriptsize
\centering
% \resizebox{\columnwidth}{!}{ % scale to columnwidth
\resizebox{0.8\textwidth}{!}{
\setlength{\tabcolsep}{0.8mm}
\begin{tabular}{|l|c|c|c
|c >{\columncolor{bgcolor}}c c >{\columncolor{bgcolor}}c
|c >{\columncolor{bgcolor}}c c >{\columncolor{bgcolor}}c
|}

\hline
    \textbf{Approach}
    & \textbf{\scriptsize{GT}}
    & \textbf{\scriptsize{GT}} 
    & \textbf{Align}
    & \multicolumn{4}{c|}{\textbf{\staticthings{}}}
    & \multicolumn{4}{c|}{\textbf{\blendedmvs{}}}
    \\

    & \textbf{\scriptsize{Poses}}
    & \textbf{\scriptsize{Range}}
    &
    & $\absrel\downarrow$ & $\threshI\uparrow$ & $\ause\downarrow$ & time [s]
    & $\absrel\downarrow$ & $\threshI\uparrow$ & $\ause\downarrow$ & time [s]
    \\
    \hline
    \hline

    \textbf{a) Classical:}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\

    \textsc{Colmap}~\cite{Schoenberger2016MVS,Schoenberger2016SfM}
    & \my
    & \mn
    & \mn
	& {5.8}
	& {79.5}
	& -
	& $\approx\SI{2}{\minute}$
	& {1.4}
	& {97.2}
	& -
	& $\approx\SI{2}{\minute}$
	\\ % colmap000002

	\textsc{Colmap} \scriptsize{Dense}~\cite{Schoenberger2016MVS,Schoenberger2016SfM}
	& \my
	& \mn
	& \mn
	& 16.6
	& 65.7
	& -
	& $\approx\SI{2}{\minute}$
	& 4.2
	& 92.3
	& -
	& $\approx\SI{2}{\minute}$
	\\ % colmap000001
	
\hline
\hline

    \textbf{b)}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\

	DeMoN~\cite{Ummenhofer2016}
	& \mn
	& \mn
	& $\Vert \vect t \Vert$
	& 36.4
	& 6.3
	& -
	& {0.07}
	& {34.4}
	& {14.5}
	& -
	& {0.08}
	\\ % demon000003

	DeepV2D \scriptsize{\scannet{}}\normalsize{~\cite{Teed2020Deepv2d}}
	& \mn
	& \mn
	& med
	& {23.1}
	& {15.4}
	& -
	& 2.73
	& -
	& -
	& -
	& -
	\\ % deepv2d_000005

	DeepV2D \scriptsize{\kitti{}}\normalsize{\cite{Teed2020Deepv2d}}
	& \mn
	& \mn
	& med
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	\\ % deepv2d_000006
	
\hline
\hline

    \textbf{c)}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\

	MVSNet~\cite{Yao2018}
	& \my
	& \my
	& \mn
	& 38.9
	& 39.0
	& 0.45
	& 0.06
	& 5.0
	& 80.7
	& 0.30
	& {0.03}
	\\ % mvsnet000007

	MVSNet Inv. Depth~\cite{Yao2018}
	& \my
	& \my
	& \mn
	& 26.5
	& 43.3
	& 0.59
	& 0.12
	& 46.1
	& 14.8
	& 0.38
	& 0.07
	\\ % mvsnet000015

	Vis-MVSNet~\cite{Zhang2020}
	& \my
	& \my
	& \mn
	& 10.4
	& {59.3}
	& {0.42}
	& 0.47
	& {2.5}
	& {92.6}
	& {0.20}
	& 0.47
	\\ % vis_mvsnet000010

	CVP-MVSNet \normalsize{~\cite{Yang2020}}
	& \my
	& \my
	& \mn
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	& {-}
	\\ % cvp_mvsnet000006

	PatchmatchNet~\cite{Wang2020}
	& \my
	& \my
	& \mn
	& {7.6}
	& 58.1
	& 0.58
	& 0.07
	& 22.1
	& 27.9
	& 0.43
	& 0.05
	\\ % patchmatchnet000001

	Fast-MVSNet~\cite{Yu2020}
	& \my
	& \my
	& \mn
	& 24.9
	& 42.7
	& 0.52
	& 0.26
	& 13.0
	& 59.2
	& 0.45
	& 0.11
	\\ % fast_mvsnet000003

	MVS2D \scriptsize{\dtu{}}\normalsize{~\cite{Yang2022}}
	& \my
	& \my
	& \mn
	& 88.3
	& 2.6
	& 0.52
	& {0.04}
	& 38.9
	& 7.3
	& 0.54
	& 0.04
	\\ % mvs2d_000004

	MVS2D \scriptsize{\scannet{}}\normalsize{~\cite{Yang2022}}
	& \my
	& \my
	& \mn
	& {39.9}
	& {2.7}
	& -
	& {0.04}
	& {64.3}
	& {1.6}
	& -
	& {0.04}
	\\ % mvs2d_000001
	
\hline
\hline

    \textbf{d) Absolute scale:}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\
    
	DeMoN~\cite{Ummenhofer2016}
	& \my
	& \mn
	& \mn
	& 36.3
	& 6.2
	& -
	& 0.08
	& 44.2
	& 7.6
	& -
	& 0.08
	\\ % demon000004

	DeepTAM~\cite{Zhou2018}
	& \my
	& \mn
	& \mn
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	\\ % deeptam000001

	DeepV2D \scriptsize{\kitti{}}\normalsize{~\cite{Teed2020Deepv2d}}
	& \my
	& \mn
	& \mn
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	\\ % deepv2d_000007

	DeepV2D \scriptsize{\scannet{}}\normalsize{~\cite{Teed2020Deepv2d}}
    & \my
    & \mn
    & \mn
	& 86.2
	& 1.8
	& -
	& 1.92
	& -
	& -
	& -
	& -
	\\ % deepv2d_000003

	MVSNet \normalsize{~\cite{Yao2018}}
    & \my
    & \mn
    & \mn
	& 26.1
	& 42.2
	& {0.48}
	& 0.12
	& -
	& -
	& -
	& -
	\\ % mvsnet000010

	MVSNet Inv. Depth\normalsize{~\cite{Yao2018}}
	& \my
	& \mn
	& \mn
	& 53.4
	& 4.7
	& -
	& 0.14
	& {29.1}
	& 48.7
	& -
	& 0.07
	\\ % mvsnet000014

	CVP-MVSNet \normalsize{~\cite{Yang2020}}
	& \my
	& \mn
	& \mn
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	\\ % cvp_mvsnet000007

	Vis-MVSNet~\cite{Zhang2020}
    & \my
    & \mn
    & \mn
	& 9.6
	& 59.2
	& 0.39
	& 0.47
	& -
	& -
	& -
	& -
	\\ % vis_mvsnet000012

	PatchmatchNet~\cite{Wang2020}
    & \my
    & \mn
    & \mn
	& 42.5
	& 2.6
	& 0.36
	& {0.04}
	& 44.7
	& {8.4}
	& {0.38}
	& 0.06
	\\ % patchmatchnet000002

	Fast-MVSNet~\cite{Yu2020}
    & \my
    & \mn
    & \mn
	& {26.1}
	& {35.9}
	& -
	& 0.21
	& 174.5
	& 15.8
	& -
	& 0.19
	\\ % fast_mvsnet000002

	MVS2D \scriptsize{\scannet{}}\normalsize{~\cite{Yang2022}}
    & \my
    & \mn
    & \mn
	& 92.4
	& 0.0
	& -
	& {0.04}
	& 29.9
	& {52.3}
	& -
	& {0.05}
	\\ % mvs2d_000003

	MVS2D \scriptsize{\dtu{}}\normalsize{~\cite{Yang2022}}
    & \my
    & \mn
    & \mn
	& 97.2
	& {0.0}
	& 0.02
	& 0.04
	& 45.6
	& 21.1
	& 0.19
	& {0.04}
	\\ % mvs2d_000006

	{Robust MVD Baseline}
    & \my
    & \mn
    & \mn
	& {6.3}
	& 54.7
	& 0.19
	& 0.04
	& {3.4}
	& 81.4
	& 0.20
	& 0.04
	\\ % distnet000178

\hline
\end{tabular}
}
\caption{\textbf{Quantitative results on \staticthings{} and \blendedmvs{} test sets.} Results are reported for the \absrelname{} ($\absrel$), the \threshIname{} ($\threshI$) with a threshold of $1.25$, the \ausename{} ($\ause$) and the model runtime in seconds. Results are for the quasi-optimal selection of \otherviews{}. \textsc{COLMAP} results are not directly comparable due to a lower prediction density.
\label{tab:eval_baseline_traindata}
}
\end{table*}
% \end{table}


==> tables/eval_baselines_merged.tex <==
\begin{table*}[t!]
% \begin{table}[t]
\footnotesize
\centering
% \resizebox{\columnwidth}{!}{ % scale to columnwidth
% \resizebox*{\textwidth}{!}{
\setlength{\tabcolsep}{2mm}
\begin{tabular}{|l
|c >{\columncolor{bgcolor}}c
|c >{\columncolor{bgcolor}}c
|c >{\columncolor{bgcolor}}c
|c >{\columncolor{bgcolor}}c
|c >{\columncolor{bgcolor}}c
|c >{\columncolor{bgcolor}}c c
|}

\hline
    \textbf{Approach}
    & \multicolumn{2}{c|}{\textbf{\kittishort{}}}
    & \multicolumn{2}{c|}{\textbf{\scannetshort{}}}
    & \multicolumn{2}{c|}{\textbf{\ethdshort{}}}
    & \multicolumn{2}{c|}{\textbf{\dtushort{}}}
    & \multicolumn{2}{c|}{\textbf{\tanksandtemplesshort{}}}
    & \multicolumn{3}{c|}{\textbf{Average}}
    \\

    & $\absrel\downarrow$ & $\threshI\uparrow$
    & $\absrel\downarrow$ & $\threshI\uparrow$
    & $\absrel\downarrow$ & $\threshI\uparrow$
    & $\absrel\downarrow$ & $\threshI\uparrow$
    & $\absrel\downarrow$ & $\threshI\uparrow$
    & $\absrel\downarrow$ & $\threshI\uparrow$ & time [ms] $\downarrow$
    \\
    \hline
    \hline
    
    \textbf{a) Depth-from-video}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\
    
	DeMoN~\cite{Ummenhofer2016}
	& 15.5
	& 75.2
	& {12.0}
	& {83.8}
	& {17.4}
	& {75.1}
	& 21.9
	& 81.2
	& 13.0
	& 83.6
	& {16.0}
	& {79.8}
	& {76.0}
	\\ % demon000003
    
    \ttodo{DeepTAM}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\
    
	DeepV2D (\scannet{})~\cite{Teed2020Deepv2d}
	& {10.0}
	& {87.6}
	& {4.4}
	& {98.1}
	& -
	& -
	& {7.7}
	& {93.8}
	& {9.4}
	& {89.7}
	& -
	& -
	& -
	\\ % deepv2d_000005
    
	DeepV2D (\kitti{})~\cite{Teed2020Deepv2d}
	& {3.1}
	& {98.5}
	& {23.5}
	& {64.9}
	& {26.8}
	& {57.7}
	& {24.5}
	& {57.6}
	& {33.8}
	& {52.8}
	& {22.3}
	& {66.3}
	& {13509.5}
	\\ % deepv2d_000006
    
    \ttodo{Neural RGB-D}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\

\hline
\hline
    
    \textbf{b) Depth-from-video GT poses}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\
    
	DeMoN~\cite{Ummenhofer2016}
	& {16.7}
	& {73.3}
	& 75.0
	& 0.8
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	& -
	& {-}
	\\ % demon000004

	DeepV2D (\scannet{})~\cite{Teed2020Deepv2d}
	& {57.9}
	& {20.3}
	& {4.1}
	& {98.3}
	& {16.1}
	& {78.2}
	& {8.4}
	& {92.1}
	& {35.4}
	& {46.0}
	& {24.4}
	& {67.0}
	& {-}
	\\ % deepv2d_000003
	
	DeepV2D (\kitti{})~\cite{Teed2020Deepv2d}
	& {20.4}
	& {81.6}
	& {25.8}
	& {55.7}
	& {30.1}
	& {55.9}
	& {24.6}
	& {56.7}
	& {38.5}
	& {54.1}
	& {27.9}
	& {60.8}
	& {19483.9}
	\\ % deepv2d_000007

\hline
\hline
    
    \textbf{c) Multi-view stereo}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\

	MVSNet (\dtu{})~\cite{Yao2018, Yao2020}
	& 22.8
	& 80.6
	& 24.6
	& 68.3
	& 35.4
	& 70.9
	& 1.8
	& {98.6}
	& {8.3}
	& {91.2}
	& {18.6}
	& {81.9}
	& {154.6}
	\\ % mvsnet000005

	Vis-MVSNet~\cite{Zhang2020}
	& {9.5}
	& {93.0}
	& {8.9}
	& {92.2}
	& {10.8}
	& {88.4}
	& {1.8}
	& 97.8
	& {4.1}
	& {95.7}
	& {7.0}
	& {93.4}
	& 734.9
	\\ % vis_mvsnet000002
    
    \ttodo{CVP-MVSNet}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\
    
    \ttodo{DPS-Net}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\
    
    \ttodo{COLMAP}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\

\hline
\hline
    
    \textbf{d) Multi-view stereo range [0.4, 100]}
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
	& 
    \\

	MVSNet (\dtu{})~\cite{Yao2018, Yao2020}
	& 14.3
	& 83.7
	& 1701.6
	& 29.5
	& 540.8
	& 32.2
	& 4073.4
	& 0.5
	& 108.9
	& 75.0
	& 1287.8
	& 44.2
	& {171.7}
	\\ % mvsnet000006

	Vis-MVSNet~\cite{Zhang2020}
	& {10.3}
	& {92.1}
	& {139.3}
	& {59.4}
	& {60.1}
	& {52.0}
	& {847.5}
	& {8.7}
	& {22.9}
	& {85.8}
	& {216.0}
	& {59.6}
	& 1938.4
	\\ % vis_mvsnet000003

\hline
\hline
    
    \textbf{e) Robust MVS Baseline}
	& {9.3}
	& {91.2}
	& {8.0}
	& {93.3}
	& {13.3}
	& {84.8}
	& {4.0}
	& {96.3}
	& {9.1}
	& {93.9}
	& {8.7}
	& {91.9}
	& {108.0}
	\\ % distnet000112


\hline
\end{tabular}
\caption{Quantitative results of our zero-shot cross-domain evaluation.
\label{tab:eval_components_merged}
}
\end{table*}
% \end{table}


==> tables/eval_relative_scale.tex <==
% \begin{table*}[t!]
\begin{table}[h!]
\footnotesize
\centering
% \resizebox{\columnwidth}{!}{ % scale to columnwidth
% \resizebox*{\textwidth}{!}{
\setlength{\tabcolsep}{0.5mm}
\begin{tabular}{|l
|c 
|c 
|c 
|c 
|c 
|c 
|}

\hline
    \textbf{Approach}
    & \textbf{\kittishort{}}
    & \textbf{\scannetshort{}}
    & \textbf{\ethdshort{}}
    & \textbf{\dtushort{}}
    & \textbf{\tanksandtemplesshort{}}
    & \textbf{Average}
    \\
    \hline
    \hline

	DeMoN~\cite{Ummenhofer2016}
	& 15.5
	& 12.0
	& 17.4
	& 21.9
	& 13.0
	& 16.0
	\\ % demon000003
	
	DeepV2D \scriptsize{\kitti{}}\normalsize{\cite{Teed2020Deepv2d}}
	& \trainedsimto{\bestresult{3.1}}
	& {23.5}
	& {26.8}
	& 24.5
	& 33.8
	& {22.3}
	\\ % deepv2d_000006

	DeepV2D \scriptsize{\scannet{}}\normalsize{~\cite{Teed2020Deepv2d}}
	& 10.0
	& \trainedsimto{\bestresult{4.4}}
	& 11.9
	& 7.7
	& 9.4
	& 8.7
	\\ % deepv2d_000005

	MVSNet \normalsize{~\cite{Yao2018}}
	& 22.8
	& 24.6
	& 35.4
	& \trainedsimto{1.8}
	& 8.3
	& 18.6
	\\ % mvsnet000007
	
	CVP-MVSNet \normalsize{~\cite{Yang2020}}
	& 156.7
	& 133.9
	& 159.0
	& \trainedsimto{{4.0}}
	& {26.1}
	& 95.9
	\\ % cvp_mvsnet000006

	Vis-MVSNet~\cite{Zhang2020}
	& 9.5
	& 8.9
	& 10.8
	& \trainedsimto{\bestresult{1.8}}
	& \bestresult{4.1}
	& 7.0
	\\ % vis_mvsnet000010

	Robust MVD Baseline
	& \bestresult{7.1}
	& \bestresult{7.4}
	& \bestresult{9.0}
	& \bestresult{2.7}
	& 5.0
	& \bestresult{6.3}
	\\ % distnet000178

\hline
\end{tabular}
\caption{\textbf{Evaluation with a relative scale, as common in literature.} Predicted depth maps of depth-from-video methods are aligned to the ground truth based on the medians. Multi-view stereo models are provided with minimum and maximum depth values of the ground truth. Results are reported with the \absrelname{} for the quasi-optimal selection of \otherviews{}. Results in parentheses denote that the model was trained on data from the same domain. Bold denotes best results among models that were not trained on data from the same domain. All models perform significantly better on the respective training domain. Note that the \baselinename{} is evaluated without re-scaling.
\label{tab:eval_baseline_relative_scale}
}
% \end{table*}
\end{table}

